Few-Shot Segmentation with Global and Local Contrastive Learning

In this work, we address the challenging task of few-shot segmentation. Previous few-shot segmentation methods mainly employ the information of support images as guidance for query image segmentation. Although some works propose to build cross-reference between support and query images, their extraction of query information still depends on the support images. We here propose to extract the information from the query itself independently to benefit the few-shot segmentation task. To this end, we first propose a prior extractor to learn the query information from the unlabeled images with our proposed global-local contrastive learning. Then, we extract a set of predetermined priors via this prior extractor. With the obtained priors, we generate the prior region maps for query images, which locate the objects, as guidance to perform cross interaction with support features. In such a way, the extraction of query information is detached from the support branch, overcoming the limitation by support, and could obtain more informative query clues to achieve better interaction. Without bells and whistles, the proposed approach achieves new state-of-the-art performance for the few-shot segmentation task on PASCAL-5$^{i}$ and COCO datasets.

==> Tables/sota_coco_bk.tex <==
\begin{table*}
\centering
\caption{1-shot and 5-shot mIoU results on COCO dataset. The results of CANet* is obtained from~\cite{pmm}.} 
\centering
\label{sota_coco}
\resizebox{1\linewidth}{!}{
\begin{tabular}{c|c|c|cccc|c|cccc|c}
\toprule[1.5pt]
{}                          & {}                                & {}                           & \multicolumn{5}{c|}{{1-shot}}                                                                                                       & \multicolumn{5}{c}{{5 shot}}                                                                                                       \\ \cline{4-13} 
\multirow{-2}{*}{{Methods}} & \multirow{-2}{*}{{Training Size}} & \multirow{-2}{*}{{Backbone}} & {Fold-0} & {Fold-1} & {Fold-2} & {Fold-3} & {Mean}          & {Fold-0} & {Fold-1} & {Fold-2} & {Fold-3} & {Mean}          \\  \midrule[0.5pt]
PANet    &     417 $\times$ 417          & VGG 16     & -     & -                              & -    & -     & 20.9    & -    & -    & -    & -     & 29.7 \\ 
FWBF     & {512 $\times$ 512}      & {VGG 16}                        & {18.4}   & {16.7}   & {19.6}   & {25.4}   & {20.0}          & {20.9}   & {19.2}   & {21.9}   & {28.4}   & {22.6}          \\ 
PFENet                      & {473 $\times$ 473}                       & {VGG 16}                       & 33.4 & 36.0 & 34.1 & 32.8 & 34.1  & 35.9 & 40.7 & 38.1 & 36.1 & 37.7   \\
\midrule[0.5pt]
{Ous}                      & {321  $\times$ 321}                       & {VGG 16}                      &32.2 &35.2 &32.2 &31.9 &32.8     
&33.8 &38.5 &37.3 &36.4 &36.5        \\
{Ous}                      & {473  $\times$ 473}                       & {VGG 16}                        &32.4 &38.1 &35.7 &32.7 & 34.7         &33.4 &42.2 &39.5 &37.6 &38.2          \\

\midrule[0.5pt] \midrule[0.5pt]

CANet*  & 321 $\times$ 321     & ResNet 50  & 25.1  & 30.3                           & 24.5 & 24.7  & 26.1    & 26.0 & 32.4 & 26.1 & 27.0 & 27.9 \\ 
PMMs   &   321 $\times$ 321  & ResNet 50  & 29.5  & 36.8 & 29.0 & 27.0  & 30.6    & 33.8 & 42.0 & 33.0 & 33.3  & 35.5 \\ 

PPNet    & -    & ResNet 50    & 28.1 & 30.8 & 29.5 & 27.7 & 29.0 & 39.0 & 40.8 & 37.1 & 37.3 & 38.5  \\
                
RPMM    &   321 $\times$ 321 & ResNet 50      & 29.5 & 36.8 & 28.9 & 27.0 & 30.6  & 33.8 & 42.0 & 33.0 & 33.3 & 35.5   \\    
                
PFENet     &  473 $\times$ 473                       &  ResNet 50   & 36.5 & 38.6 & {34.5} & {33.8} & {35.8} & 36.5 & 43.3 & 37.8 & 38.4 & 39.0 \\   

\midrule[0.5pt] 

{Ous}                      & {321 X 321}                       & {ResNet 50}                        &34.4 &38.5 &34.6 &33.2 & 35.2        &38.9 &46.2 &39.1 &38.9 & 40.7          \\

Ours    &  473  $\times$ 473       & ResNet 50  & {36.7}  & {41.4}                           & {38.7} & {36.6}  & {38.3}    & {41.5} & {48.1} & {46.3} & {43.6}  & {44.8} \\

\midrule[0.5pt] \midrule[0.5pt]

DAN  & -    & ResNet 101  & - & - & - & - & 24.4 & - & - & - & - & 29.6  \\
FWBF      &    512 $\times$ 512  & ResNet 101 & 19.9  & 18.0    & 21.0 & 28.9  & 21.2    & 19.1 & 21.5 & 23.9 & 30.1  & 23.7 \\ 
PFENet   & 641 $\times$ 641     & ResNet 101 & 34.3  & 33.0 & 32.3 & 30.1  & 32.4    & 38.5 & 38.6 & 38.2  & 34.3  & 37.4 \\ 
\midrule[0.5pt] \midrule[0.5pt]

% Ours    &  473  $\times$ 473       & ResNet 50  & {36.7}  & {41.4}                           & {38.7} & {36.6}  & {38.3}    & {41.5} & {48.1} & {46.3} & {43.6}  & {44.8} \\

{Ous}                      & {321  $\times$ 321}                       & {ResNet 101}                       &33.0 &38.4 &36.8 &32.8 & 35.2         &38.9 &46.7 &43.1 &40.4 & 42.3          \\
{Ous}                      & {473  $\times$ 473}                       & {ResNet 101}                       &39.0 &42.6 &40.5 &40.2 & 40.5        &43.8 &46.8 &47.5 &42.6 & 45.2       \\

\bottomrule[1.5pt]
% Ours    &  641 $\times$ 641      & ResNet 50  & 35.81 & 39.12                          & 37.8 & 35.76 & 37.1225 & -    & -    & -    & -     & -    \\ 
\end{tabular}
}
\vspace{+0.46cm}
\end{table*}



==> Tables/sota_coco_simple.tex <==
\begin{table*}
\centering
\caption{1-shot and 5-shot mIoU results on COCO dataset. The results of CANet* is obtained from~\cite{pmm}. The results reported with mIoU(\%)} 
\centering
\label{sota_coco}
\resizebox{1\linewidth}{!}{
\begin{tabular}{c|c|c|cccc|c|cccc|c}
\toprule[1.5pt]
{}                          & {}                                & {}                           & \multicolumn{5}{c|}{{1-shot}}                                                                                                       & \multicolumn{5}{c}{{5 shot}}                                                                                                       \\ \cline{4-13} 
\multirow{-2}{*}{{Methods}} & \multirow{-2}{*}{{Training Size}} & \multirow{-2}{*}{{Backbone}} & {Fold-0} & {Fold-1} & {Fold-2} & {Fold-3} & {Mean}          & {Fold-0} & {Fold-1} & {Fold-2} & {Fold-3} & {Mean}          \\  \midrule[0.5pt]
PANet   &     417 $\times$ 417          & VGG 16     & -     & -                              & -    & -     & 20.9    & -    & -    & -    & -     & 29.7 \\ 
FWBF      & {512 $\times$ 512}      & {VGG 16}                        & {18.4}   & {16.7}   & {19.6}   & {25.4}   & {20.0}          & {20.9}   & {19.2}   & {21.9}   & {28.4}   & {22.6}          \\ 
PFENet                      & {473 $\times$ 473}                       & {VGG 16}                       & 33.4 & 36.0 & 34.1 & 32.8 & 34.1  & 35.9 & 40.7 & 38.1 & 36.1 & 37.7   \\
\midrule[0.5pt]
% {Ous}                      & {473  $\times$ 473}                       & {VGG 16}                        & {-}   & {-}   & {-}   & {-}   & {-}          & {-}   & {-}   & {-}   & {-}   & {-}          \\
% {Ous}                      & {321  $\times$ 321}                       & {VGG 16}                        & {-}   & {-}   & {-}   & {-}   & {-}          & {-}   & {-}   & {-}   & {-}   & {-}          \\
% \midrule[0.5pt] \midrule[0.5pt]

CANet  & 321 $\times$ 321     & ResNet 50  & 25.1  & 30.3                           & 24.5 & 24.7  & 26.1    & 26.0 & 32.4 & 26.1 & 27.0 & 27.9 \\ 
PMMs    &   321 $\times$ 321  & ResNet 50  & 29.5  & 36.8 & 29.0 & 27.0  & 30.6    & 33.8 & 42.0 & 33.0 & 33.3  & 35.5 \\ 

PPNet   & -    & ResNet 50    & 28.1 & 30.8 & 29.5 & 27.7 & 29.0 & 39.0 & 40.8 & 37.1 & 37.3 & 38.5  \\
                
RPMM  &   321 $\times$ 321 & ResNet 50      & 29.5 & 36.8 & 28.9 & 27.0 & 30.6  & 33.8 & 42.0 & 33.0 & 33.3 & 35.5   \\    
                
PFENet      &  473 $\times$ 473                       &  ResNet 50   & 36.5 & 38.6 & {34.5} & {33.8} & {35.8} & 36.5 & 43.3 & 37.8 & 38.4 & 39.0 \\   

\midrule[0.5pt] 

% {Ous}                      & {321 X 321}                       & {ResNet 50}                        &34.4 &38.5 &34.6 &33.2 & 35.2        &38.9 &46.2 &39.1 &38.9 & 40.7          \\

% Ours    &  473  $\times$ 473       & ResNet 50  & \textbf{36.7}  & \textbf{41.4}                           & \textbf{38.7} & \textbf{36.6}  & \textbf{38.3}    & \textbf{41.5} & \textbf{48.1} & \textbf{46.3} & \textbf{43.6}  & \textbf{44.8} \\

% \midrule[0.5pt] \midrule[0.5pt]

DAN  & -    & ResNet 101  & - & - & - & - & 24.4 & - & - & - & - & 29.6  \\
FWBF     &    512 $\times$ 512  & ResNet 101 & 19.9  & 18.0    & 21.0 & 28.9  & 21.2    & 19.1 & 21.5 & 23.9 & 30.1  & 23.7 \\ 
PFENet  & 641 $\times$ 641     & ResNet 101 & 34.3  & 33.0 & 32.3 & 30.1  & 32.4    & 38.5 & 38.6 & 38.2  & 34.3  & 37.4 \\ 
\midrule[0.5pt] \midrule[0.5pt]


% {Ous}                      & {321  $\times$ 321}                       & {ResNet 101}                        & {-}   & {-}   & {-}   & {-}   & {-}          & {-}   & {-}   & {-}   & {-}   & {-}          \\
% {Ous}                      & {321  $\times$ 321}                       & {ResNet 101}                        & {-}   & {-}   & {-}   & {-}   & {-}          & {-}   & {-}   & {-}   & {-}   & {-}        \\
{Ous}                      & {321 X 321}                       & {ResNet 50}                        &34.4 &38.5 &34.6 &33.2 & 35.2        &38.9 &46.2 &39.1 &38.9 & 40.7          \\

Ours    &  473  $\times$ 473       & ResNet 50  & \textbf{36.7}  & \textbf{41.4}                           & \textbf{38.7} & \textbf{36.6}  & \textbf{38.3}    & \textbf{41.5} & \textbf{48.1} & \textbf{46.3} & \textbf{43.6}  & \textbf{44.8} \\


\bottomrule[1.5pt]
% Ours    &  641 $\times$ 641      & ResNet 50  & 35.81 & 39.12                          & 37.8 & 35.76 & 37.1225 & -    & -    & -    & -     & -    \\ 
\end{tabular}
}
\vspace{+.36cm}
\end{table*}


